Sequencer Level Security

Current blockchains do not provide any security guarantees to the smart contracts and their users as far as the content of the transactions is concerned. In the spirit of decentralization and censorship resistance, they follow the paradigm of including valid transactions in blocks without any further scrutiny. Rollups are a special kind of blockchains whose primary purpose is to scale the transaction throughput. Many of the existing rollups operate through a centrally operated sequencing protocol. In this paper, we introduce the Sequencer Level Security (SLS) protocol, an enhancement to sequencing protocols of rollups. This pioneering contribution explores the concept of the sequencer's capability to identify and temporarily quarantine malicious transactions instead of including them in blocks immediately. We describe the mechanics of the protocol for both the transactions submitted to the rollup mempool, as well as transactions originating from Layer one. We comment on topics such as trust and decentralization, and consider the security impact on the protocol itself. We implement a prototype of the SLS protocol, Zircuit, which is built on top of Geth and the OP stack. The SLS protocol described can be easily generalized to other rollup designs, and can be used for purposes other than security.

==> old/inclusion-deposit-transaction.tex <==
%%% jgorzny: Previously section 4.4

\subsection{Inclusion of a Deposit Transaction in a block}
As described before, deposit transactions are picked up from the L1 to be later included in a block. However, this process is not performed by \texttt{op-geth}. It is instead carried out by \texttt{op-node}. 
\texttt{op-node} provides information to \texttt{op-geth} regarding the current tip of the chain. This process happens thanks to an endpoint of the ``engine'' API of geth that exposes the \texttt{forkchoiceUpdated} set of methods. %, namely: \texttt{forkchoiceUpdatedV1}, \texttt{forkchoiceUpdatedV2} and \texttt{forkchoiceUpdatedV3}. %%%% jgorzny: the specific names are never reused; lets leave them out
Through these methods, \texttt{op-node} communicates the current Head, Safe, and Finalized blocks\todo{JG: These types are not defined} to \texttt{op-geth} and together with these it can include a set of payload attributes that contain the deposit transactions derived from the L1. 
If the call includes payload attributes, \texttt{op-geth} makes a new block that includes the transactions in the payload.

==> sections/evaluation.tex <==
\section{Evaluation}\label{sec:evaluation}


\todo[inline]{Coming soon; planned in 3508.}


==> sections/introOld.tex <==
\section{Introduction}\label{sec:intro}


Smart contracts deployed on blockchain networks often manage assets of financial value. 
In this paper, we are concerned with the security guarantees that networks offer to smart contracts. The Ethereum protocol, in the spirit of absolute censorship resistance, does not put any scrutiny on the transactions before including them in blocks—the block proposers are able to include any properly signed and priced transactions, regardless of what they execute on-chain.\todo{JG: what is a ``properly priced transaction''?} 
This is no different for current rollups. 
In this paper, we introduce a novel concept of Sequencer Level Security for rollups with centralized sequencers. 
A sequencer that implements this protocol considers the effect that transactions have on-chain, and if it is undesirable, it temporarily prevents transactions from being executed. 
This provides the smart contract operators and users with an opportunity to take mitigation steps before suffering harm. 
The presented protocol does not impact the level of censorship resistance of rollups with centralized sequencers. This paper does not focus on the analysis of transactions themselves (we defer the curious reader to Section~\ref{sec:related} for results in the detection area), but rather on the capability to use the results by the sequencing protocol itself.

We describe the concept in the setting of an Ethereum rollup based on the architecture of Optimism, and its implementation via the OP stack framework and Geth.\todo{MD from doc: how do I say it will be implemented on Zircuit?}
However, the concept can be easily generalized to other rollups with centralized sequencers, and blockchains other than Ethereum. 

The paper is organized as follows. 
Following this introduction, Section \ref{sec:prelim} describes the preliminaries of the Ethereum and Optimism Bedrock. 
Section \ref{sec:sls} contains the main contribution of this paper and introduces the sequencing protocol with enhanced security. 
In Section \ref{sec:implementation}, we confirm implementation viability and address implementation concerns for a rollup built using the OP stack framework. We conclude in Section \ref{sec:conclusion}.

